SegGPT: Segmenting Everything In Context

We present SegGPT, a generalist model for segmenting everything in context. We unify various segmentation tasks into a generalist in-context learning framework that accommodates different kinds of segmentation data by transforming them into the same format of images. The training of SegGPT is formulated as an in-context coloring problem with random color mapping for each data sample. The objective is to accomplish diverse tasks according to the context, rather than relying on specific colors. After training, SegGPT can perform arbitrary segmentation tasks in images or videos via in-context inference, such as object instance, stuff, part, contour, and text. SegGPT is evaluated on a broad range of tasks, including few-shot semantic segmentation, video object segmentation, semantic segmentation, and panoptic segmentation. Our results show strong capabilities in segmenting in-domain and out-of-domain targets, either qualitatively or quantitatively.

==> figures/teaser.tex <==




\makeatletter
\let\@oldmaketitle\@maketitle%
\renewcommand{\@maketitle}{\@oldmaketitle%
\vspace{-2em}
    \centering
    \includegraphics[width=.96\linewidth]{figures/seggpt_teaser.pdf}
    \captionof{figure}{\Ours is capable of segmenting everything in context \textit{with only 
    \textbf{one single}
    model}, %
    which uses 
    in-context examples %
    to 
    indicate different tasks. For each sample, the orange box \textcolor{orange}{$\square$} on the left displays the example/prompt image and its corresponding mask, while the blue box \textcolor{cyan}{$\square$}  on the right shows the input image and the resulting mask output. The mask represents the bright region attached to the image. The caption for each sample (in the yellow box) is only for explanation. Notably, \Ours can perform arbitrary object segmentation (segment different components of the scene, such as the big red sphere, all the spheres, contour of all spheres, top surfaces, and shadows), multiple part segmentation (specialized parts of the iconic Statue of Liberty), rainbow segmentation, video object segmentation without videos in training, and close-set semantic segmentation with learnable prompt tuning. More examples are shown in Figure~\ref{fig:vis_2}.
    }
    \label{fig:teaser}
   \bigskip}                   %
\makeatother




